Jiamusi pulsar observations: III. Nulling of 20 pulsars

Most of pulsar nulling observations were conducted at frequencies lower than 1400~MHz. We aim to understand the nulling behaviors of pulsars at relatively high frequency, and to check if nulling is caused by a global change of pulsar magnetosphere. 20 bright pulsars are observed at 2250~MHz with unprecedented lengths of time by using Jiamusi 66m telescope. Nulling fractions of these pulsars are estimated, and the null and emission states of pulses are identified. Nulling degrees and scales of the emission-null pairs are calculated to describe the distributions of emission and null lengths. Three pulsars, PSRs J0248+6021, J0543+2329 and J1844+00, are found to null for the first time. The details of null-to-emission and emission-to-null transitions within pulse window are first observed for PSR J1509+5531, which is a small probability event. A complete cycle of long nulls for hours is observed for PSR J1709-1640. For most of these pulsars, the K-S tests of nulling degrees and nulling scales reject the hypothesis that null and emission are of random processes at high significance levels. Emission-null sequences of some pulsars exhibit quasi-periodic, low-frequency or featureless modulations, which might be related to different origins. During transitions between emission and null states, pulse intensities have diverse tendencies for variations. Significant correlations are found for nulling fraction, nulling cadence and nulling scales with the energy loss rate of the pulsars. Combined with the nulling fractions reported in literatures for 146 nulling pulsars, we found that statistically large nulling fractions are more tightly related to pulsar period than to characteristic age or energy loss rate.

==> fig_sci.tex <==

\begin{figure*}
  \begin{tabular}{l}
    \includegraphics[bb = 25 40 282 182, clip, height=0.155\textheight] {B0329+54_201602211028_ds.ps} 
    \includegraphics[bb = 50 40 489 182, clip, height=0.155\textheight] {B0329+54_201602241326_ds.ps} \\
    \includegraphics[bb = 25 40 530 182, clip, height=0.155\textheight] {B0329+54_201711081846_ds.ps} \\
%  \end{tabular}
%  \begin{tabular}{c}
    \includegraphics[bb = 32 32 280 272, clip, height=0.15\textheight] {B0329+54_201602211028_AC.ps} 
    \includegraphics[bb = 65 32 280 272, clip, height=0.15\textheight] {B0329+54_201602241326_AC.ps}
    \includegraphics[bb = 65 32 320 272, clip, height=0.15\textheight] {B0329+54_201711081846_AC.ps}
   \end{tabular}
  \caption{The dynamic spectra $S(\nu,t)$ from three observations of
    PSR B0329+54 ({\it upper three panels}) and their auto-correlation
    functions $A(\Delta \nu,\Delta t)$ ({\it three panels in the
      lowest rank}). Some dummy points caused by the interference are
    shown as $S(\nu,t)=0$. The pulsar name and observation time in MJD
    are indicated in each plot. The auto-correlation functions are
    plotted against time lag $\Delta t$ in minutes and frequency lag
    $\Delta \nu$ in MHz, and the two-dimensional Gaussian fitting are
    shown only in the cross-section for $\Delta \nu =0$ and $\Delta t
    =0$ plotted in the side-panels. The color schemes are saturated at
    $-10$\% and 60\% of the peak values as indicated by the wedge.}
  \label{fig0329}
\end{figure*}

\begin{figure*}
  \begin{tabular}{l}
    \includegraphics[bb = 25 40 510 182, clip, angle=0, height=0.155\textheight] {B0355+54_201508202106_ds.ps}
    \includegraphics[bb = 50 40 166 182, clip, angle=0, height=0.155\textheight] {B0355+54_201601292120_ds.ps}\\
    \includegraphics[bb = 25 40 529 182, clip, angle=0, height=0.155\textheight] {B0355+54_201601290850_ds.ps}
    \includegraphics[bb = 488 40 510 182, clip, angle=0, height=0.155\textheight] {B0355+54_201508202106_ds.ps}\\
    \includegraphics[bb = 25 40 400 182, clip, angle=0, height=0.155\textheight] {B0355+54_201711060010_ds.ps}
    \includegraphics[bb = 50 40 400 182, clip, angle=0, height=0.155\textheight] {B0355+54_201711091756_ds.ps}\\
    %
    \includegraphics[bb = 32 32 279 272, clip,angle=0, height=0.154\textheight] {B0355+54_201508202106_AC.ps}
    \includegraphics[bb = 65 32 279 272, clip,angle=0, height=0.154\textheight] {B0355+54_201601292120_AC.ps} 
    \includegraphics[bb = 65 32 279 272, clip,angle=0, height=0.154\textheight] {B0355+54_201601290850_AC.ps}
    \includegraphics[bb = 65 32 279 272, clip,angle=0, height=0.154\textheight] {B0355+54_201711060010_AC.ps}
    \includegraphics[bb = 65 32 320 272, clip,angle=0, height=0.154\textheight] {B0355+54_201711091756_AC.ps}\\
    %
 %   \includegraphics[bb = 32 32 330 270, clip,angle=0, height=0.125\textheight] {B0355+54_201508202106_SS.ps}
 %    \includegraphics[bb = 70 32 330 270, clip,angle=0, height=0.125\textheight] {B0355+54_201601292120_SS.ps}
 %    \includegraphics[bb = 70 32 330 270, clip,angle=0, height=0.125\textheight] {B0355+54_201601290850_SS.ps}
 %    \includegraphics[bb = 70 32 330 270, clip,angle=0, height=0.125\textheight] {B0355+54_201711060010_SS.ps}
 %    \includegraphics[bb = 70 32 370 270, clip,angle=0, height=0.125\textheight] {B0355+54_201711091756_SS.ps}   
  \end{tabular}
  \caption{Dynamic spectra from five observations of PSR B0355+54
    ({\it upper five panels}) and the autocorrelation functions ({\it
      the second last rank of panels}). See keys in
    Fig.~\ref{fig0329}. The secondary spectra are plotted against
    conjugate time and frequency ({\it bottom rank of panels}), which
    are logarithmic in spectral power. The dashed curves represent the
    best fitting to arcs.  }
  \label{fig0355}
\end{figure*}

\begin{figure*}
%  \begin{tabular}{l}
    \includegraphics[bb = 25 40 119 182, clip, angle=0, height=0.155\textheight] {B0540+23_201506251100_ds.ps}
    \includegraphics[bb = 50 40 231 182, clip, angle=0, height=0.155\textheight] {B0540+23_201608090445_ds.ps} 
    \includegraphics[bb = 50 40 430 182, clip, angle=0, height=0.155\textheight] {B0540+23_201711012106_ds.ps} \\
    %
    \includegraphics[bb = 32 32 279 272, clip, angle=0, height=0.154\textheight] {B0540+23_201506251100_AC.ps}
    \includegraphics[bb = 65 32 279 272, clip, angle=0, height=0.154\textheight] {B0540+23_201608090445_AC.ps}
    \includegraphics[bb = 65 32 320 272, clip, angle=0, height=0.154\textheight] {B0540+23_201711012106_AC.ps}\\
    %
  %  \includegraphics[bb = 32 32 330 270, clip, angle=0, height=0.127\textheight] {B0540+23_201506251100_SS.ps}
  %  \includegraphics[bb = 70 32 330 270, clip, angle=0, height=0.127\textheight] {B0540+23_201608090445_SS.ps}
  %  \includegraphics[bb = 70 32 370 270, clip, angle=0, height=0.127\textheight] {B0540+23_201711012106_SS.ps} 
%  \end{tabular}
  \caption{Dynamic spectra from three observations of PSR B0540+23
    ({\it upper panels}) and the autocorrelation functions ({\it
      middle panels}) and secondary spectra ({\it bottom 
      panels}). See keys in Fig.~\ref{fig0355}.}
  \label{fig0540}
\end{figure*}


\begin{figure*}
    \includegraphics[bb = 25 40 243 182, clip, angle=0, height=0.155\textheight] {B0740-28_201512120030_ds.ps} 
    \includegraphics[bb = 50 40 256 182, clip, angle=0, height=0.155\textheight] {B0740-28_201601262105_ds.ps} 
    \includegraphics[bb = 50 40 260 182, clip, angle=0, height=0.155\textheight] {B0740-28_201711020255_ds.ps} \\ 
    \includegraphics[bb = 32 32 279 272, clip, angle=0, height=0.154\textheight] {B0740-28_201512120030_AC.ps}
    \includegraphics[bb = 65 32 279 272, clip, angle=0, height=0.154\textheight] {B0740-28_201601262105_AC.ps}
    \includegraphics[bb = 65 32 320 272, clip, angle=0, height=0.154\textheight] {B0740-28_201711020255_AC.ps}
  \caption{Dynamic spectra from three observations of PSR B0740-28
    ({\it upper panels}) and autocorrelation functions ({\it lower
      panels}). See keys in Fig.~\ref{fig0329}. }
  \label{fig0740}
\end{figure*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}
  \includegraphics[bb = 25 40 205 182, clip,angle=0, height=0.155\textheight] {B1508+55_201512140350_ds.ps}
  \includegraphics[bb = 50 40 152 182, clip,angle=0, height=0.155\textheight] {B1508+55_201710310630_ds.ps}\\
  \includegraphics[bb = 32 32 279 272, clip,angle=0, height=0.154\textheight] {B1508+55_201512140350_AC.ps}
  \includegraphics[bb = 65 32 320 272, clip,angle=0, height=0.154\textheight] {B1508+55_201710310630_AC.ps} 
  \caption{Dynamic spectra from two observations of PSR B1508+55 ({\it
      upper panels}) and autocorrelation functions ({\it lower
      panels}). See keys in Fig.~\ref{fig0329}. }
  \label{fig1508}
\end{figure}






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure*}
  \centering
  \begin{tabular}{l}
    \includegraphics[bb = 25 40 93  172, clip, angle=0, height=0.155\textheight] {B1933+16_201506160205_ds.ps}
    \includegraphics[bb = 50 40 332 172, clip, angle=0, height=0.155\textheight] {B1933+16_201602190440_ds.ps} \\
    \includegraphics[bb = 25 40 527 172, clip, angle=0, height=0.155\textheight] {B1933+16_201602260440_ds.ps} \\
    \includegraphics[bb = 25 40 370 172, clip, angle=0, height=0.155\textheight] {B1933+16_201605210150_ds.ps} \\
    \includegraphics[bb = 25 40 505 172, clip, angle=0, height=0.155\textheight] {B1933+16_201605212310_ds.ps} \\
    \includegraphics[bb = 25 40 505 172, clip, angle=0, height=0.155\textheight] {B1933+16_201605222340_ds.ps} \\
    \includegraphics[bb = 25 40 385 172, clip, angle=0, height=0.155\textheight] {B1933+16_201605240125_ds.ps}
    \includegraphics[bb = 50 40 225 172, clip, angle=0, height=0.155\textheight] {B1933+16_201605260210_ds.ps}
  \end{tabular}
  \caption{Dynamic spectra from eight observations of PSR
    B1933+16. See keys in Fig.~\ref{fig0329}.}
  \label{fig1933DS}
\end{figure*}
%
\begin{figure*}
  \centering
  \begin{tabular}{l}
    \includegraphics[bb = 32 62 279 272, clip, angle=0, height=0.131\textheight] {B1933+16_201506160205_AC.ps}
    \includegraphics[bb = 67 62 279 272, clip, angle=0, height=0.131\textheight] {B1933+16_201602190440_AC.ps}
    \includegraphics[bb = 67 62 279 272, clip, angle=0, height=0.131\textheight] {B1933+16_201602260440_AC.ps}
    \includegraphics[bb = 67 62 320 272, clip, angle=0, height=0.131\textheight] {B1933+16_201605210150_AC.ps} \\
    \includegraphics[bb = 32 32 279 272, clip, angle=0, height=0.15\textheight] {B1933+16_201605212310_AC.ps}
    \includegraphics[bb = 67 32 279 272, clip, angle=0, height=0.15\textheight] {B1933+16_201605222340_AC.ps}
    \includegraphics[bb = 67 32 279 272, clip, angle=0, height=0.15\textheight] {B1933+16_201605240125_AC.ps}
    \includegraphics[bb = 67 32 279 272, clip, angle=0, height=0.15\textheight] {B1933+16_201605260210_AC.ps}
  \end{tabular}
  \caption{The autocorrelation functions of dynamic spectra for eight
    observations of PSR B1933+16. See keys in Fig.~\ref{fig0329}.}
  \label{fig1933AC}
\end{figure*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure*}
  \begin{tabular}{l}
    \includegraphics[bb = 25 40 220 182, clip, angle=0, height=0.155\textheight] {B2154+40_201601251455_ds.ps} 
    \includegraphics[bb = 50 40 302 182, clip, angle=0, height=0.155\textheight] {B2154+40_201710312035_ds.ps}
    \includegraphics[bb = 50 40 290 182, clip, angle=0, height=0.155\textheight] {B2154+40_201711101140_ds.ps} 
  \end{tabular}
  \begin{tabular}{c}
    \includegraphics[bb = 32 32 279 272, clip, angle=0, height=0.154\textheight] {B2154+40_201601251455_AC.ps}
    \includegraphics[bb = 64 32 279 272, clip, angle=0, height=0.154\textheight] {B2154+40_201710312035_AC.ps}
    \includegraphics[bb = 64 32 320 272, clip, angle=0, height=0.154\textheight] {B2154+40_201711101140_AC.ps}
  \end{tabular}
 % \begin{tabular}{c}
 %   \includegraphics[bb = 32 32 330 270, clip, angle=0, height=0.127\textheight] {B2154+40_201601251455_SS.ps}
 %   \includegraphics[bb = 65 32 330 270, clip, angle=0, height=0.127\textheight] {B2154+40_201710312035_SS.ps}
 %   \includegraphics[bb = 65 32 370 270, clip, angle=0, height=0.127\textheight] {B2154+40_201711101140_SS.ps} 
 % \end{tabular}
  \caption{Dynamic spectra ({\it upper three panels}), autocorrelation
    functions ({\it middle three panels}) and secondary spectra ({\it
      bottom three panels}) for three observations of PSR
    B2154+40. See keys in Fig.~\ref{fig0329}.  }
  \label{fig2154}
\end{figure*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}
  \begin{tabular}{l}
    \includegraphics[bb = 25 40 250 182, clip, angle=0, height=0.152\textheight] {B2310+42_201507202135_ds.ps} \\
    \includegraphics[bb = 25 40 400 182, clip, angle=0, height=0.152\textheight] {B2310+42_201710252101_ds.ps} \\
    \includegraphics[bb = 32 32 279 272, clip, angle=0, height=0.154\textheight] {B2310+42_201507202135_AC.ps}
    \includegraphics[bb = 65 32 320 272, clip, angle=0, height=0.154\textheight] {B2310+42_201710252101_AC.ps}
  \end{tabular}
  \caption{Dynamic spectra from two observations of PSR B2310+42 ({\it
      upper two panels}) and the autocorrelation functions ({\it lower
      two panels}). See keys in Fig.~\ref{fig0329}. }
  \label{fig2310}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}
  \begin{tabular}{l}
    \includegraphics[bb = 25 40 250 182, clip, angle=0, height=0.152\textheight] {B2324+60_201703291426_ds.ps} \\
    \includegraphics[bb = 25 40 400 182, clip, angle=0, height=0.152\textheight] {B2324+60_201711041040_ds.ps} \\
    \includegraphics[bb = 32 32 279 272, clip, angle=0, height=0.154\textheight] {B2324+60_201703291426_AC.ps}
    \includegraphics[bb = 64 32 320 272, clip, angle=0, height=0.154\textheight] {B2324+60_201711041040_AC.ps}
  \end{tabular}
  \caption{Dynamic spectra from two observations of PSR B2324+60 ({\it
      upper two panels}) and the autocorrelation functions ({\it lower
      two panels}). See keys in Fig.~\ref{fig0329}. }
  \label{fig2324}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}
  \centering
  \begin{tabular}{l}
    \includegraphics[bb = 25 40 128 182, clip, angle=0, height=0.143\textheight] {B2351+61_201506190015_ds.ps}
    \includegraphics[bb = 51 40 200 182, clip, angle=0, height=0.143\textheight] {B2351+61_201608110515_ds.ps} \\
%    \includegraphics[bb = 50 40 213 182, clip, angle=0, height=0.143\textheight] {B2351+61_201710292116_ds.ps} 
%    \includegraphics[bb = 50 40 358 182, clip, angle=0, height=0.143\textheight] {B2351+61_201710292350_ds.ps}
%  \end{tabular}
%  \begin{tabular}{c}
    \includegraphics[bb = 32 32 279 272, clip, angle=0, height=0.154\textheight] {B2351+61_201506190015_AC.ps}
    \includegraphics[bb = 64 32 279 272, clip, angle=0, height=0.154\textheight] {B2351+61_201608110515_AC.ps}
%    \includegraphics[bb = 64 32 279 272, clip, angle=0, height=0.154\textheight] {B2351+61_201710292116_AC.ps}
 %   \includegraphics[bb = 64 32 320 272, clip, angle=0, height=0.154\textheight] {B2351+61_201710292350_AC.ps}
  \end{tabular}
  \caption{Dynamic spectra from four observations of PSR B2351+61
    ({\it upper panels}) and the autocorrelation functions ({\it
      lower panels}). See keys in Fig.~\ref{fig0329}.}
  \label{fig2351}
\end{figure}








==> figure.tex <==














